Bridging Data-Driven and Knowledge-Driven Approaches for Safety-Critical Scenario Generation in Automated Vehicle Validation

Automated driving vehicles~(ADV) promise to enhance driving efficiency and safety, yet they face intricate challenges in safety-critical scenarios. As a result, validating ADV within generated safety-critical scenarios is essential for both development and performance evaluations. This paper investigates the complexities of employing two major scenario-generation solutions: data-driven and knowledge-driven methods. Data-driven methods derive scenarios from recorded datasets, efficiently generating scenarios by altering the existing behavior or trajectories of traffic participants but often falling short in considering ADV perception; knowledge-driven methods provide effective coverage through expert-designed rules, but they may lead to inefficiency in generating safety-critical scenarios within that coverage. To overcome these challenges, we introduce BridgeGen, a safety-critical scenario generation framework, designed to bridge the benefits of both methodologies. Specifically, by utilizing ontology-based techniques, BridgeGen models the five scenario layers in the operational design domain (ODD) from knowledge-driven methods, ensuring broad coverage, and incorporating data-driven strategies to efficiently generate safety-critical scenarios. An optimized scenario generation toolkit is developed within BridgeGen. This expedites the crafting of safety-critical scenarios through a combination of traditional optimization and reinforcement learning schemes. Extensive experiments conducted using Carla simulator demonstrate the effectiveness of BridgeGen in generating diverse safety-critical scenarios.

==> 04_3_design.tex <==
% 3.3
\section{The Scenario Generation Algorithm Toolkit}\label{sec:GenerationAlgorithm}


% 5.2
\subsection{Intelligent Evaluation of Autonomous Vehicles}
In the development of autonomous driving technology, extensive testing, evaluation, and validation are required. In particular, emphasis must be placed on an autonomous vehicle's decision-making ability and perception of complex environments. Researching methods for evaluating the intelligence of autonomous vehicles provides higher feedback to generate algorithms for key scenarios, forming a closed-loop iterative optimization. However, there is currently no unified standard for evaluating the intelligence of autonomous vehicles. Different evaluation indicators and methods have been proposed for different application scopes. This section introduces the key aspects of autonomous vehicle evaluation and constructs a target function based on evaluation indicators.
% 5.2.1
\subsubsection{Evaluation Indicators for Key Aspects}\label{sec:Evaluation Indicators for Key Aspects}
Scenarios are constructed through generative algorithm searches, and target functions are built using evaluation indicators to score the scenarios. Feedback is then provided to the generative algorithms for continuous adjustment of the search direction, forming a closed-loop iterative optimization. The design of evaluation indicators is thus crucial, with a focus on key indicators for evaluating autonomous driving scenarios~\cite{sun2021scenario}.

The purpose of key indicators is to detect high-risk, boundary, and collision scenarios. Indicators include: collision or not, the minimum distance with different traffic participants, and the speed at that minimum distance, etc.

% 5.2.2
\subsubsection{Objective Function Design}\label{sec:Objective Function Design}
The objective function, as the optimization target for the generative algorithm, must reflect the overall testing goals and requirements objectively. It should have certain continuity to quantify the importance of each scenario parameter combination and effectively apply the generative algorithm. Constraints based on ODD and naturalness indicators can exclude invalid scenarios, and objective function attributes are selected, such as the minimum distance between the ego and background vehicles and the corresponding speed of the ego vehicle when at this minimum distance.

After determining the intelligence evaluation indicators for autonomous vehicles, appropriate evaluation methods need to be chosen. In the evaluation system, multiple indicators exist, so a balanced optimization needs to be achieved for multi-objective optimization algorithms. For single-objective optimization algorithms, a combined index evaluation method is required to determine the evaluation results of the evaluation object on different indicators. This method explains the different aspects of the evaluated object with multiple evaluation indicators and finally synthesizes the results of each indicator, using a total index to illustrate the overall level of the evaluated object. This method also requires further determination of index weights after establishing the index system.

The method of determining index weights can be divided into subjective weighting and objective weighting. Subjective weighting is based on expert judgment, and the analytic hierarchy process is commonly used. Objective weighting is derived from mathematical calculations and analyses of actual index attribute values, thus obtaining weight coefficients, with entropy weighting being more common. Objective weighting uses more refined mathematical models and methods, free from human influence, but depends on data, and the index weight changes with the evaluated object, lacking universality.

Therefore, the combination weighting method is adopted, finding the most reasonable weight coefficients within both subjective and objective weighting, with the former accounting for 40\% and the latter 60\%, finally obtaining a comprehensive evaluation weight coefficient. This method reflects both subjective information and original data to some extent, giving the weight coefficient objectivity.

This paper uses random algorithms to generate test data, and based on this data, adopts the combination weighting method to determine the weight of each evaluation indicator to construct the objective function. This serves as the default weight in the evaluation system for each indicator. Additionally, one may modify the designated evaluation indicator weight according to specific needs. By calculating the randomly generated data, the weight ratio between two target attributes, the minimum distance between the main and background vehicles (min\_distance\_vehicle) and the corresponding speed of the main vehicle at this minimum distance (speed\_vehicle), is determined to be 0.8297:0.1703. Therefore, the target value for the single-objective optimization algorithm, \(fit\), is as follows:
% equation 7
\begin{equation}
    fit = -0.8297 \times \text{min\_distance\_vehicle} + 0.1703 \times \text{speed\_vehicle}
    \label{eq:7}
\end{equation}

% 5.2.3
\subsubsection{Key Test Scenario Identification Method}\label{sec:Key Test Scenario Identification Method}
Currently, there is no general consensus on key scenarios. Zhang et al.~\cite{xinxin2020csg} describe key scenarios as dangerous road situations that may cause autonomous vehicles to make unsafe decisions and that must be immediately countered to avoid imminent collisions. Gambi et al.~\cite{gambi2019generating} use accident scenarios from police reports as key test scenarios for autonomous vehicles, while Klischat et al.~\cite{klischat2019generating} believe that human driver accidents are not necessarily key scenarios and can be avoided by others or autonomous vehicles. One component of key scenario identification is how to quantify and evaluate whether a specific scenario is key or non-key, so the key nature of a scenario must be expressed in a quantifiable way.

This paper uses the evaluation indicators proposed in \ref{sec:Evaluation Indicators for Key Aspects} and the objective function in \ref{sec:Objective Function Design} to classify scenario keyness. It quantitatively identifies key scenarios using collision status, minimum distance between the main vehicle and traffic participants, and speed at that minimum distance~\cite{song2022critical}. TTC represents the remaining time before a collision if the vehicle maintains its current speed and direction. A shorter TTC means a higher likelihood of collision, and a smaller minimum distance or a greater speed at that minimum distance indicates a more dangerous scenario. Table~\ref{tab:Threshold Values} shows the threshold values for classifying key scenarios for each evaluation indicator:

% table 3
\begin{table}[]
\caption{Threshold Values for Key Scenario Classification Based on Evaluation Indicators}
\centering
\setlength\tabcolsep{18pt}  % adjusting table width (optional)
\begin{tabular}{c|c}
\toprule
    \textbf{Evaluation Indicator} & \textbf{Threshold for Key Scenario}   \\ 
\midrule
    $n_{collision}$ & $ \textgreater 0$ \\ 
    $d_{min}$ & $ \textless 2$ \\ 
    $v_d$  & $\geq 1$  \\
\bottomrule
\end{tabular}
\label{tab:Threshold Values}
\end{table}


The ratio of the \textbf{key scenario proportion} found by the two algorithms is NSGA-\uppercase\expandafter{\romannumeral2}-DT:RS=0.649:0.541. The key scenario proportion of NSGA-\uppercase\expandafter{\romannumeral2}-DT is greater than that of RS. \textbf{As shown in the figure}, the distribution of the target attribute values of the NSGA-\uppercase\expandafter{\romannumeral2}-DT algorithm's scenarios is roughly the same as that of the RS algorithm's scenarios, but as the iterations progress, the optimization effect of the target attributes of the scenarios generated by the NSGA-\uppercase\expandafter{\romannumeral2}-DT algorithm is better, that is, minimizing the minimum distance between the main car and the background vehicles and maximizing the speed of the main car corresponding to the minimum distance. Moreover, the \textbf{key scenario generation time} of the RS algorithm is 1.567 times that of NSGA-\uppercase\expandafter{\romannumeral2}-DT, demonstrating that the NSGA-\uppercase\expandafter{\romannumeral2}-DT algorithm is more efficient than the RS algorithm in terms of search efficiency.


The \textbf{average frequency distribution} of different objective functions obtained by the NSGA-\uppercase\expandafter{\romannumeral2}-DT algorithm and RS algorithm for the generated scenarios \textbf{is shown in the figure}, ...


\textbf{Hypervolume Indicator (HV)} is a comprehensive index for evaluating the convergence and diversity of approximate solution sets, ...


\textbf{Spread Evaluation} is mainly used to measure the non-uniformity of the non-inferior solution set, ...


